Neurodiversity in Computing Education Research: A Systematic Literature Review

Ensuring equitable access to computing education for all students-including those with autism, dyslexia, or ADHD-is essential to developing a diverse and inclusive workforce. To understand the state of disability research in computing education, we conducted a systematic literature review of research on neurodiversity in computing education. Our search resulted in 1,943 total papers, which we filtered to 14 papers based on our inclusion criteria. Our mixed-methods approach analyzed research methods, participants, contribution types, and findings. The three main contribution types included empirical contributions based on user studies (57.1%), opinion contributions and position papers (50%), and survey contributions (21.4%). Interviews were the most common methodology (75% of empirical contributions). There were often inconsistencies in how research methods were described (e.g., number of participants and interview and survey materials). Our work shows that research on neurodivergence in computing education is still very preliminary. Most papers provided curricular recommendations that lacked empirical evidence to support those recommendations. Three areas of future work include investigating the impacts of active learning, increasing awareness and knowledge about neurodiverse students' experiences, and engaging neurodivergent students in the design of pedagogical materials and computing education research.

==> archive/old-discussion.tex <==
\subsection{Educational Opportunities}


\subsubsection{Active Learning}

As mentioned in our results, one paper mentioned that with the increasingly common shift towards active learning in computing courses, it may inadvertently introduce new barriers to computing education for neurodivergent students who experience social difficulties~\cite{pilotte2016autism}.
In recent years, there has been increased interest in moving towards more active learning in computing courses~\cite{mccartney2017folk} due to their benefits, such as improved student outcomes~\cite{greer2019effects} and student retention~\cite{latulipe2018evolving}. However, a lot of research remains unexplored about how active learning impacts neurodivergent students, positively or negatively. It is important that researchers engage with neurodivergent students to design versions of these pedagogical techniques which are more inclusive for all students.

\subsubsection{Informal Education}
In our review, we only identified one paper which discussed informal learning with autistic college students~\cite{begel2021remote}. Prior CER for neurodivergent K-12 learners has found informal learning to be beneficial for students' programming self-efficacy~\cite{kokinda2024informal}, teamwork and collaboration~\cite{moster2022can}, and interest in computing~\cite{wang2023virtual}. We see informal educational experiences as a key opportunity area for future research to explore for neurodivergent post-secondary computing students.

\subsubsection{Accessibility Education}
There has been a large push to include more accessibility education in computing courses~\cite{elglaly2024beyond, zhao2020comparison, shinohara2018teaches, baker2020systematic}. Researchers have begun to develop curricula and materials to support accessibility education to integrate it within the computing education curriculum beyond human-computer interaction courses~\cite{elglaly2024beyond, kuang2024mapping}. Accessibility and disability is a large and highly diverse research area~\cite{mack2021we}. As highlighted by Kletenik et al.~\cite{kletenik2024awareness} and corroborated by the results of our study, there is a need for more research into how to incorporate neurodiversity-centered accessibility education in computing courses to not only inform students but create greater awareness about neurodiversity for university faculty and staff. 

\subsection{Methodological Considerations for Future Research}
As we note in the results, we found that, of the 14 papers we analyzed, 57.1\% of them contained the results of empirical studies. When compared to a broader view of CER which found that approximately 80\% of papers published in CER venues (e.g., TOCE, SIGCSE, ITiCSE) contained some form of empirical data~\cite{heckman2021systematic}, this highlights a key opportunity to conduct more empirical research about the experiences and preferences of neurodivergent students in computing. 

The amount of neurodiversity-centered CER is trending in the right direction (see Figure~\ref{fig:year-of-pub}), and we encourage researchers and practitioners to consider to explore this important emerging field of work. When doing so, however, it is important to report thoroughly on our research in order to produce high-quality research~\cite{heckman2021systematic}. This includes providing clear research goals and questions, study materials, and clear description of methodology. Responsible research about neurodivergence and accessibility should also follow the tenet, ``nothing about us without us''~\cite{charlton1998nothing, williams2019nothing}, as much as possible, meaning, whenever possible, researchers should include the populations they are researching in the research process. Including neurodivergent students in future research will be vital in conducting high-quality, equitable research~\cite{burke2022students}. The papers we analyzed often framed the traits of neurodivergent students as challenges or deficits to be overcome, and we encourage researchers to adopt a social model of disability, rather than a medical model which frames disability as something to be fixed~\cite{marks1997models}, focusing on ways in which existing systems can be changed to provide adequate support and services for neurodivergent students~\cite{oliver1990individual} through strategies like access grafting~\cite{borsotti2024neurodiversity}.
